Chemical Evolution with Radial Mixing Redux: Extending beyond the Solar Neighborhood

We present a multi-zone galactic chemical evolution (GCE) model for the Milky Way that takes the most recently updated yields of major nucleosynthesis channels into account. It incorporates physical processes commonly found in previous GCE models like supernova and star formation feedback, the radial flow of gas in the disk, and the infall of fresh gas, along with stellar scattering processes like radial migration. We individually analyse the effect of different physical processes present in our model on the observed properties of the Galaxy. The radial flow of gas in the disk plays an important role in establishing the radial gradient for \feh{} in the low-\alphafe{} sequence. Our model with one episode of smooth gas infall and constant star formation efficiency is capable of reproducing the observed \fehalpha{} distribution of stars at different ($R$, $|z|$) positions in the Milky Way. Our results point to the rapid evolution of \alphafe{} after the onset of Type Ia supernovae and a high star formation rate during the formation of the high-\alphafe{} sequence as the origin of dual peaks in \alphafe{}. A secondary infall is unnecessary to reproduce the \alphafe{}-gap and chemical spread in the disk in our model. We additionally compare the median age for various mono-abundance populations and the age-metallicity relation at different ($R$, $|z|$) positions from our fiducial model to observations. We discuss our results in relation to other related work in detail.

==> dump.tex <==
We depart from \cite{2009MNRAS.396..203S} and adopt a different radial inflow mechanism. However, as radial inflow significantly impacts the chemical tracks, we briefly describe their mechanism here and implement it for the purpose of comparison. It iterates from the innermost to the outermost zone, each zone grabbing fresh gas from the IGM and existing cold gas from the next zone. The exact amount from the IGM is determined by $M_{n, IGM, t} = (f_A+f_B) \times \Delta M_{n, t} + f_B \times M_{n-1, n, t}$ where $M_{n-1, n, t}$ is the mass that moves from zone $n-1$ to zone $n$ through radial inflow. The radial inflow mass makes up for the rest of $ \Delta M_{n, t}$ and thus $M_{n, n+1, t} = \Delta M_{n, t} - M_{n, IGM, t}$. The innermost zone only receives gas so its IGM equation does not have a radial inflow term. 

They compared three scenarios,  scheme A ($f_A \neq 0$, $f_B = 0$), scheme B ($f_A=0$, $f_B \neq 0$) and scheme AB ($f_A \neq 0$, $f_B \neq 0$). In scheme A, each zone fetches a fixed fraction of $\Delta M_{n, t}$ so $M_{n-1, n, t}$ can be readily calculated as $\sum_{i=0}^{n-1} f_A \Delta M_{i, t}$. The sum monotonically increases and causes radial mass influx to build up towards the outskirts of the galaxy. Scheme B allows additional mass to be fetched from the IGM in each zone and thus significantly reduces the radial mass influx in the outer zones. Scheme AB has an intermediate effect, while the actual values involved do not the equal the sum of those from scheme A and B with the same specified $f_A$ and $f_B$. We found that certain values of $f_A$ and $f_B$ caused all of the cold ISM in some outer zones to be transferred inwards.

\begin{figure*}
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{figures/tracks_MgFe_v_FeH_GALAH.pdf} % first figure itself
        \caption{first figure}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1.2\textwidth]{figures/tracks_MgFe_v_FeH_GALAH.pdf} % second figure itself
        \caption{second figure}
    \end{minipage}
\end{figure*}

\begin{align} \label{eq:sfr}
    \frac{d\Sigma_*}{dt} = C
    \begin{cases}
            \Sigma_{{g}}^{1.4} & \Sigma_{{g}} > \Sigma_{{crit}}\\
            \Sigma_{{crit}}^{-2.6}\Sigma_{{g}}^{4} & o.w.
    \end{cases}
\end{align}
